SugarCrepe: Fixing Hackable Benchmarks for Vision-Language Compositionality

In the last year alone, a surge of new benchmarks to measure compositional understanding of vision-language models have permeated the machine learning ecosystem. Given an image, these benchmarks probe a model's ability to identify its associated caption amongst a set of compositional distractors. Surprisingly, we find significant biases in all these benchmarks rendering them hackable. This hackability is so dire that blind models with no access to the image outperform state-of-the-art vision-language models. To remedy this rampant vulnerability, we introduce SugarCrepe, a new benchmark for vision-language compositionality evaluation. We employ large language models, instead of rule-based templates used in previous benchmarks, to generate fluent and sensical hard negatives, and utilize an adversarial refinement mechanism to maximally reduce biases. We re-evaluate state-of-the-art models and recently proposed compositionality inducing strategies, and find that their improvements were hugely overestimated, suggesting that more innovation is needed in this important direction. We release SugarCrepe and the code for evaluation at: https://github.com/RAIVNLab/sugar-crepe.

==> sections/08-checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
   \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
   \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
   \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/img2txt_retrieval_with_hns.tex <==
% \begin{table*}[t]
%      \centering
%      \caption{Following existing compositionality benchmarks for vision-language models, \method adopts image-to-text retrieval for evaluation, where the query is an image and the retrieval set consists of one positive caption plus (at least) one composition-aware hard negative text. }
%      \resizebox{\textwidth}{!}{
%      {\renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lllll}
% \small
% \textbf{Image}     & \multicolumn{4}{l}{\textbf{Text retrieval set}}                                                                                                              \\ 
%          \multirow{8}{*}{\includegraphics[width=0.3\textwidth]{imgs/img_example.jpg}}          & \multicolumn{3}{l}{Positive}                                   & \positive{Set of toy animals sitting in front of a red wooden wagon.}                         \\\cline{2-5}
%                    &                                 &                           & Object    & \negative{Balloons} sitting in front of a red wooden wagon.                                   \\
%                    &                                 &                           & Attribute & Set of \negative{real} animals sitting in front of a red wooden wagon. \\
%                    &                                 & \multirow{-3}{*}{Replace} & Relation  & Set of toy animals \negative{inside} a red wooden wagon.                                      \\\cline{3-5}
%                    &                                 &                           & Object    & \negative{Red wooden wagon} sitting in front of a \negative{set of toy animals}.                         \\
%                    &                                 & \multirow{-2}{*}{Swap}    & Attribute & Set of \negative{wooden} animals sitting in front of a red \negative{toy} wagon.                         \\\cline{3-5}
%                    &                                 &                           & Object    & \negative{Flowers} and a set of toy animals are sitting in front of a red wooden wagon.       \\
% \multirow{-8}{*}{} & \multirow{-7}{*}{Hard Negative} & \multirow{-2}{*}{Add}     & Attribute & A \negative{mechanical} set of toy animals sitting in front of a red wooden wagon. \\\cline{2-5}          
% \end{tabular}}}
% \label{tab:img2txt_retrieval}
% \end{table*}
  

==> tables/linear_probe.tex <==
\begin{table*}[t]
	\small{
    \centering
    \begin{tabular}{cccccccccc}
    \small
    \shortstack[c]{Pretraining\\ Dataset} &
    \shortstack[c]{Method} &
    \rotatebox{65}{\footnotesize{Caltech101}} &
    \rotatebox{65}{\footnotesize{Food101}} &
    \rotatebox{65}{\footnotesize{Sun397}} &
    \rotatebox{65}{\footnotesize{Flowers102}} & 
    \rotatebox{65}{\footnotesize{CUB}} &
    \rotatebox{65}{\footnotesize{Stanford Cars}} &
    \rotatebox{65}{\footnotesize{FGVC Aircraft}} &
    \rotatebox{65}{\footnotesize{Average}}\\
    \toprule
    \multirow{5}{*}{CC3M}     & CYCLIP~\cite{goel2022cyclip} & 80.88 & 54.95 & - & 83.74 & - & 22.72 & 28.02 & -   \\
    & CLIP~\cite{RadfordKHRGASAM21} &  80.11 & 53.82 & 56.40 & 84.07 & 40.30 & 22.70 & 35.61 & 53.29\\
    & CLIP-HELIP & 82.49 & 59.79 & 59.56 & 87.84 & 46.19 & 30.01 & 42.48 & 58.34  \\
    & SLIP~\cite{MuK0X22} & 87.96 &  72.50  & 66.96  & 91.91 & 49.77 & 39.25 & 45.87 & 64.89 \\
    & SLIP-\hclip & \textbf{89.64} & \textbf{73.09} & \textbf{67.67} & \textbf{93.02} & \textbf{53.16} & \textbf{42.44}& \textbf{48.66} &  \textbf{66.81} \\
    % \cdashline{1-10}
    \midrule
    \multirow{4}{*}{CC12M}     & CLIP~\cite{RadfordKHRGASAM21} & 85.35 & 68.00 & 64.45 & 87.88 & 48.75 & 57.80 & 40.32 & 64.65 \\
    & CLIP-\hclip & 85.87 & 68.89 & 64.95 & 88.36 & 49.41 & 58.55 & 40.17 & 65.17  \\
    & SLIP~\cite{MuK0X22} & \textbf{92.89}  &  83.63  & 74.34   & 94.87 & \textbf{60.99} & 73.43 & 52.23 & 76.05 \\
    & SLIP-\hclip & 92.85 & \textbf{84.25} &\textbf{74.74} &\textbf{95.09} & 60.53 & \textbf{74.23} & \textbf{52.36} & \textbf{76.29}  \\
    % \cdashline{1-6}
    % \multirow{2}{*}{CC12M}    & CLIP & 67.41          & 85.17          & 41.06          & 59.42 \\
    %                           & Ours & \textbf{71.87} & \textbf{86.32} & \textbf{47.16} & \textbf{65.33} \\
    \bottomrule
    \end{tabular}
\vspace{1mm}
    \caption{\textbf{Linear Probe Performance on Fine-grained Image Classification.} We report the linear probe performance on a variety of classification benchmarks. In average, both the CLIP and SLIP pretrained on CC3M and CC12M are improved.}
    \label{tab:linear_probe}
	}
\end{table*}


==> tables/main_table.tex <==


\begin{table*}[h]
  \centering
  \small
  \caption{\textbf{Compositionality benchmark results:} .}
  \scalebox{0.65}{
    \begin{tabular}{ll ccccccccccc} 
    \toprule
     && \multicolumn{3}{c}{\bf Winoground} &  &\multicolumn{3}{c}{\bf CREPE}&\multicolumn{4}{c}{\bf ARO}\\ 
     \cmidrule{3-5}\cmidrule{7-9}\cmidrule{10-13}
     
    \textbf{Source} &\textbf{Model} & \textbf{Text} & \textbf{Image} & \textbf{Group} & \textbf{Cola} & \textbf{Swap} & \textbf{Atomic} & \textbf{Negate} & \textbf{VG-Relation} & \textbf{VG-Attribute} & \textbf{COCO-Order} & \textbf{Flickr30K-Order} \\ 
    \midrule

\multirow{2}{*}{OpenAI} & CLIP &   \\
   
& \method &       \\ \midrule

\multirow{2}{*}{LAION} & CLIP &   \\
   
& \method &       \\ \midrule

\multirow{2}{*}{DataComp} & CLIP &   \\
   
& \method &       \\ 

\bottomrule 
\end{tabular}
}
  
  \label{tab:main}

\end{table*}

==> tables/retrieval.tex <==
\begin{table*}[h]
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{Z}{>{\centering\arraybackslash}X}
\newcolumntype{W}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}

  \centering
  \small
\setlength\tabcolsep{1pt}
\renewcommand{\arraystretch}{1.0}
    
    \begin{tabularx}{\textwidth}{l c ZZZ c ZZZ c ZZZ c ZZZ} 
    \toprule
     &~~~&
     \multicolumn{7}{c}{\bf Text Retrieval}    &~~~~~& \multicolumn{7}{c}{\bf Image Retrieval}   \\ %
    
    \cmidrule{3-9}\cmidrule{11-17}
     
    && \multicolumn{3}{c}{\bf Flickr30k} && \multicolumn{3}{c}{\bf COCO} && \multicolumn{3}{c}{\bf Flickr30k} && \multicolumn{3}{c}{\bf COCO} \\ 
    
    \cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}

\textbf{Method} && {\it R@1}& {\it R@5}& {\it R@10}    &~~~&
         {\it R@1}     & {\it R@5}     & {\it R@10}   &~~~&
         {\it R@1}      & {\it R@5}      & {\it R@10}    &~~~&
         {\it R@1} & {\it R@5}     & {\it R@10}   \\ \midrule

CLIP &  \\ 
  
\method &       \\ \bottomrule 
\end{tabularx}

  \caption{\textbf{Retrieval results:} When performing image and text retrieval, .}
  \label{tab:retrieval}

\end{table*}
